DRAINCLoG: Detecting Rogue Accounts with Illegally-obtained NFTs using Classifiers Learned on Graphs

As Non-Fungible Tokens (NFTs) continue to grow in popularity, NFT users have become targets of phishing attacks by cybercriminals, called \textit{NFT drainers}. Over the last year, \$100 million worth of NFTs were stolen by drainers, and their presence remains a serious threat to the NFT trading space. However, no work has yet comprehensively investigated the behaviors of drainers in the NFT ecosystem. In this paper, we present the first study on the trading behavior of NFT drainers and introduce the first dedicated NFT drainer detection system. We collect 127M NFT transaction data from the Ethereum blockchain and 1,135 drainer accounts from five sources for the year 2022. We find that drainers exhibit significantly different transactional and social contexts from those of regular users. With these insights, we design \textit{DRAINCLoG}, an automatic drainer detection system utilizing Graph Neural Networks. This system effectively captures the multifaceted web of interactions within the NFT space through two distinct graphs: the NFT-User graph for transaction contexts and the User graph for social contexts. Evaluations using real-world NFT transaction data underscore the robustness and precision of our model. Additionally, we analyze the security of \textit{DRAINCLoG} under a wide variety of evasion attacks.

==> figure/ablation_study.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{Fig/ablation.pdf}
        \vspace{-0.35cm}
    \caption{
    The results of ablation experiments averaged over 10 runs. $SCE$ and $TCE$ denote social context extractor and NFT transaction context extractor, respectively. $DRAINCLoG^{-rel}$ is a modified \model{} which does not consider transaction types between users in the user graph.  }
    \label{fig:abb}
    \vspace{-0.4cm}
\end{figure}


==> figure/evasion_attack.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{Fig/finetune_attack.pdf}
      \vspace{-0.2cm}
    \caption{
    F1-score after re-updating on different cutoff dates against (a) Attack 1 and (b) Attack 2.
     Each color represents a different attack level, denoted by $L_1$ to $L_4$. 
     In Attack 2, different line types represent the varying amounts of Ether sent by the attackers. 
     For each date, the ratio of attackers to regular users was 1:100 in evaluation.}
    % The active attackers until each date are used for additional training, and the remains are used for evaluation. For each evaluation dataset, }
    \vspace{-0.2cm}
    \label{fig:finetune}
\end{figure}

==> figure/hn_ratio_discuss.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{Fig/hn_ratio_discuss.pdf}
    \caption{
    (a) The performance when varying the number of heavy users included in the training dataset.
    (b) Regular users misclassified as drainers (F.Ps) in dataset $D_4$ when heavy users are added/not added. }
    \label{fig:hn_raio}
    \vspace{-0.5cm}
\end{figure}

==> figure/holding_time.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{Fig/holding_time.pdf}
        \caption{CDFs of holding times of different user types (regular users, affiliated users, and drainers) based on out-transaction types: (a) \textit{sell} and (b) \textit{gift-out}. We include an enlarged graph for holding times smaller than a day.}
        \label{f:holding}
        \vspace{-0.2cm}
\end{figure}

==> sections/Overview.tex <==
\section{Overview}

In this section, we provide the workflow of our paper illustrated by Figure \ref{fig:overall}.
It has three main parts: \textit{Datasets Construction}, \textit{Drainer Activity Characterization}, and \textit{NFT Drainer Detection}. 
First, we construct two datasets: NFT transaction records, and drainer accounts, each collected from Ethereum blockchain and multiple websites reporting suspicious accounts (in Section \ref{sec:data}). 
% We find a few number of websites reporting suspicious Ethereum accounts including NFT drainers, but each has only 100 $\sim$ 300 addresses. Thus, it is necessary to collect NFT drainer accounts from multiple channels.
% It has not been long since NFT targeted phishing attack received attention; there investigate the of x
Then, with the above datasets, we conduct in-depth measurement study to characterize drainers activity compared to regular users along multiple dimensions (in Section \ref{sec:measurement}).
The results from the analysis provide us insights for designing and implementing our model, which consists of two modules: \firstmodule{} and \secondmodule{}. We confirm that the proposed model outperforms existing detection methods.

% User Transaction Context Extractor
% User Interaction Extractor

% Use transaction aggregation
% NFT context aggregation

% Intra NFT Transaction aggregation
% Inter NFT Transaction Context aggregation
% 유저의 NFT 거래에 집중
% 유저와 다른 유저 사이에 집중. transaction type을 고려  sale, transfer
% sale, transfer
% node - Relation Aware neighbors aggregationr
% 유저들과 어떤 관계냐 
% GCN - Topology 
 

==> table/evasion1.tex <==
\begin{table}[t]
    \caption{
    The results of the evasion attack simulation averaged over 5 runs with varying attack levels. The values listed below for Attack 2 were simulated with X = 1\%.}
    \label{tab:evasion1}
    \centering
    \footnotesize
        \begin{tabular}{l ccc |ccc}
            \toprule
            & \multicolumn{3}{c}{\textbf{Attack1}} 
            & \multicolumn{3}{c}{\textbf{Attack2}} \\
            \cmidrule{2-7}
            \multicolumn{1}{r}{Level (L\%)}
            & $D_1$ & $D_2$ & $D_3$
            & $D_1$ & $D_2$ & $D_3$ \\
            \midrule
            w/o attack &
            0.896 & 0.884 & 0.850 &
            0.896 & 0.884 & 0.850\\
            \midrule
            $L_1$ (10\%) &
            0.853 & 0.841 & 0.802 &
            0.860 & 0.848 & 0.810  \\
            $L_2$ (30\%) &
            0.775 & 0.764 & 0.726 & 
            0.790 & 0.779 & 0.742  \\
            $L_3$ (50\%) &
            0.745 & 0.733 & 0.696 & 
            0.752 & 0.741 & 0.705\\
            $L_4$ (70\%) &
            0.737 & 0.725 & 0.688 & 
            0.651 & 0.640 & 0.607  \\
            \bottomrule
        \end{tabular}
\end{table}



 




% \begin{table}[t]
%     \caption{Performance of \model{} under evasion attacks by varying the attack level ($L_1 \sim L_3$) on the datasets $D_1$ and $D_4$.}
%     \label{tab:evasion1}
%     \centering
%     \footnotesize
%         \begin{tabular}{lc ccc |ccc}
%             \toprule
%             && \multicolumn{3}{c}{\textbf{Attack1}} 
%             & \multicolumn{3}{c}{\textbf{Attack2}} \\
%             \cmidrule{3-8}
%             \multicolumn{2}{r}{Level (X\%)}
%             & Pre & Recall & F1 & Pre & Recall & F1\\
%             \midrule
%             \multirow{4}{*}{$\boldsymbol{D_1}$} 
%             & w/o (0\%)
%             & 0.921 & 0.866 & 0.889
%             & 0.921 & 0.866 & 0.889 \\
%             \cmidrule{2-8}
%             &$L_1$ (10\%) 
%             & 0.888 & 0.814 & 0.850
%             & 0.897 & 0.722 & 0.800\\            
%             &$L_2$ (20\%)
%             & 0.880 & 0.753 & 0.811
%             & 0.867	& 0.536 & 0.662\\
%             &$L_3$ (50\%)
%             & 0.868 & 0.680 & 0.763
%             & 0.758 & 0.258 & 0.385 \\
%             \midrule
%             \multirow{4}{*}{$\boldsymbol{D_4}$} 
%             & w/o (0\%)
%             & 0.562 & 0.866 & 0.681
%             & 0.562 & 0.866 & 0.681 \\
%             \cmidrule{2-8}
%             &$L_1$ (10\%) 
%             & 0.506 & 0.814 & 0.625
%             & 0.515 & 0.722 & 0.601\\            
%             &$L_2$ (20\%) 
%             & 0.487 & 0.753 & 0.591
%             & 0.441 & 0.536 & 0.484\\
%             &$L_3$ (50\%) 
%             & 0.462 & 0.680 & 0.550
%             & 0.275 & 0.258 & 0.266\\           
%             \bottomrule
%         \end{tabular}
% \end{table}





==> table/evasion2.tex <==

% \begin{table}[t]
%     \caption{Performance of \model{} under evasion attack 2.}
%     \label{tab:evasion2}
%     \centering
%     \ra{1.1}
%     \footnotesize
%         \begin{tabular}{l ccc |ccc}
%             \toprule
%             \multirow{2}{c}{\textbf{Attack 2}}
%             & \multicolumn{3}{c}{\textbf{$D_1$}} 
%             & \multicolumn{3}{c}{\textbf{$D_4$}} \\
%             \cmidrule{2-7}
%             & Pre & Recall & F1 & Pre & Recall & F1\\
%             \midrule
%             w/o attack 
%             & 0.921 & 0.866 & 0.8892
%             & 0.562 & 0.866 & 0.681  \\
%             \midrule 
%             Level 1 
%             &0.515 & 0.7216 & 0.601
%             &&&\\
%             Level 2 
%             & 0.446 & 0.639 & 0.525 \\
%             Level 3 
%             &0.412 & 0.557 & 0.474\\
%             \bottomrule
%         \end{tabular}
% \end{table}


\begin{table}[t]
    \caption{Performance of \model{} under evasion attack 1.}
    \label{tab:evasion1}
    \centering
    \ra{1.1}
    \footnotesize
        \begin{tabular}{l ccc |ccc}
            \toprule
            & \multicolumn{3}{c}{\textbf{$D_1$}} 
            & \multicolumn{3}{c}{\textbf{$D_4$}} \\
            \cmidrule{2-7}
            & Pre & Recall & F1 & Pre & Recall & F1\\
            \midrule
            w/o attack 
            & 0.921 & 0.866 & 0.8892
            & 0.921 & 0.866 & 0.8892 \\
            \midrule
            &\multicolumn{6}{c}{\textbf{Attack1}}\\
            \midrule
            Level 1 
            & & &
            & 0.462 & 0.680 & 0.550\\            
            Level 2 
            & & &
            & 0.446 & 0.639 & 0.525 \\
            Level 3 
            & & &
            &0.412 & 0.557 & 0.474\\
            \midrule
            &\multicolumn{6}{c}{\textbf{Attack2}}\\
            \midrule
            Level 1 
            & & &
            & 0.462 & 0.680 & 0.550\\            
            Level 2 
            & & &
            & 0.446 & 0.639 & 0.525 \\
            Level 3 
            & & &
            &0.412 & 0.557 & 0.474\\            
            \bottomrule
        \end{tabular}
\end{table}
 % & 0.562 & 0.866 & 0.681

==> table/event_log.tex <==
\begin{table*}[t]
% \resizebox{0.98\textwidth}{!}{
\footnotesize
\ra{1.1}
\centering
\caption{List of event logs related to NFT transfer that we collected from Ethereum blockchain.}
\begin{tabular}{lllll}
\toprule
\textbf{Contract} & \textbf{Method ID} & \textbf{Method Name} & \textbf{Description} & \textbf{Information} \\
\midrule
ERC-721 & 0xddf252ad &  \textit{transfer} & transfer of NFT standard & sender, receiver, contract address, token ID \\
CryptoPunks & 0x58e5d5a5 &  \textit{punk\_bought} & CryptoPunks token sale & sender, receiver, token ID, \textit{price} \\
CryptoPunks & 0x05af636b &  \textit{punk\_transfer} & CryptoPunks token transfer & sender, receiver, token ID\\
\bottomrule
\end{tabular}
% }

\label{tab:event_log}
\end{table*}

==> table/measurement_data_summary.tex <==
\begin{table}[h]
\caption{Summary of collected NFT transaction records. }
\label{tab:NFT_tx}
\centering
\footnotesize
\ra{1.1}
% \resizebox{\linewidth}{!}{
\begin{tabular}{l l r}
    \toprule
    \multicolumn{2}{l}{\textbf{Type}} & \textbf{Collection} \\
    \midrule
    \multicolumn{2}{l}{NFT} & 44,865,594 \\
    \multicolumn{2}{l}{Account} & 3,086,046  \\
    \multicolumn{2}{l}{Transaction} &\\

    & Mint & 45,852,904 \\
    &  Sale & 14,465,466  \\
    &    Transfer &10,482,489 \\
    &     Burn & 669,881\\ \cmidrule{2-3}
    &    Total transaction records & 71,470,740 \\
    \midrule
    \midrule
    \multicolumn{2}{l}{\textbf{Period}} &
    \multicolumn{1}{l}{January 1,2022 $\sim$ July 31, 2022}\\
    \bottomrule
\end{tabular}
%}
\end{table}



